Scale-Aware Trident Networks for Object Detection

Scale variation is one of the key challenges in object detection. In this work, we first present a controlled experiment to investigate the effect of receptive fields for scale variation in object detection. Based on the findings from the exploration experiments, we propose a novel Trident Network (TridentNet) aiming to generate scale-specific feature maps with a uniform representational power. We construct a parallel multi-branch architecture in which each branch shares the same transformation parameters but with different receptive fields. Then, we adopt a scale-aware training scheme to specialize each branch by sampling object instances of proper scales for training. As a bonus, a fast approximation version of TridentNet could achieve significant improvements without any additional parameters and computational cost compared with the vanilla detector. On the COCO dataset, our TridentNet with ResNet-101 backbone achieves state-of-the-art single-model results of 48.4 mAP. Codes are available at https://git.io/fj5vR.

==> src/experiment__Yanghao_Li_s_conflicted_copy_2019-03-20_.tex <==
\begin{section}{Experiments}\label{sec:experiment}

In this section, we conduct experiments on the COCO dataset~\cite{coco}. 
Following~\cite{bell2016inside,fpn}, we train models on the union of 80k training images and 35k subset of validation images (\textit{trainval35k}), and evaluate on a set of 5k validation images (\textit{minival}). 
We also report the final results on a set of 20k test images (\textit{test-dev}). 
We first describe the implementation details of TridentNets and training settings in Section~\ref{sec:implementation}. 
We then conduct thorough ablation experiments to validate the proposed method in Section~\ref{sec:exp_ablation}. 
Finally, Section~\ref{sec:results} compares the results of TridentNets with state-of-the-art methods on the \textit{test-dev} set.

\begin{subsection}{Implementation Details}\label{sec:implementation}
We re-implement Faster R-CNN~\cite{faster-rcnn} as our baseline method in MXNet~\cite{mxnet}. 
Following other standard detectors~\cite{rcnn,faster-rcnn}, the network backbones are pre-trained on the ImageNet~\cite{imagenet} and then finetuned on the detection dataset. 
The input images are resized to have a short side of 800 pixels. 
Both the baselines and TridentNets are trained in an end-to-end manner.
By default, we train models in a batch size of 16 on 8 GPUs. 
We train 12 epochs by default, with learning rate starting from 0.02 and decreased by a factor of 0.1 after the 8th and 10th epoch. The $2\times$ or $3\times$ training schemes means doubling or tripling the total training epochs and learning rate schedules accordingly.
We adopt the output of conv4 stage in ResNet~\cite{resnet} as the backbone feature map and conv5 stage as the rcnn head in both baseline and TridentNet. 
For each image, we sample 128 ROIs per-branch for TridentNet. 
If not otherwise specified, we adopt three branches as our default TridentNet structure.
The dilation rates are set to 1, 2 and 3 in three branches, respectively. 
When adopting scale-aware training scheme for TridentNet, we set the valid ranges of three branches as $[0, 90]$, $[30, 160]$ and $[90, \infty]$, respectively.

For the evaluation, we report the standard COCO evaluation metric of Average Precision (AP)~\cite{coco} as well as $\text{AP}_{50}$/$\text{AP}_{75}$. 
We also report COCO-style $\text{AP}_s$, $\text{AP}_m$ and $\text{AP}_l$ on objects of small (less than 32$\times$32), medium (from 32$\times$32 to 96$\times$96) and large (greater than 96$\times$96) sizes. 
\end{subsection}

\begin{subsection}{Ablation Studies}\label{sec:exp_ablation}

\begin{paragraph}{Components of TridentNet.}

\begin{table*}[hbpt]
\small
\renewcommand\arraystretch{1.25}
	\begin{center}
	\setlength{\tabcolsep}{3.5pt}
	\begin{tabular}{l|l|ccc|cc|ccc}
		\hline
		Backbone & Method & Multi-branch & Weight-sharing & Scale-aware &  AP & $\text{AP}_{50}$ & $\text{AP}_{s}$ & $\text{AP}_{m}$ & $\text{AP}_{l}$	\\
		\hline
		\multirow{5}{*}{ResNet-101} & (a) Baseline & - & - & - 					&  	37.9	& 58.8	& {20.0}& {43.0}& 52.8\\
		\cline{2-10}
			& (b) Multi-branch 	 & \checkmark &	&								&	39.0	& 59.7	& 20.6	& 43.5	& 55.1\\
			& (c) TridentNet w/o scale-aware	& \checkmark &	\checkmark	&   &	40.3    & 61.1  & 21.8	& 44.7	& \textbf{56.7}\\
			& (d) TridentNet w/o sharing & \checkmark &	&	\checkmark 			&   39.3	& 60.4	& 21.4	& 43.8	& 54.2\\
			& (e) TridentNet	& \checkmark &	\checkmark & \checkmark			&	\textbf{40.6}	& \textbf{61.8}	& \textbf{23.0} & \textbf{45.5} & 55.9 \\
		\hline	
		\multirow{5}{*}{ResNet-101-Deformable} & (a) Baseline & - & - & - 		&  	39.9    & 61.3	& 21.6  & 45.0  & 55.6\\
		\cline{2-10}
			& (b) Multi-branch  & \checkmark &	&								&	40.5	& 61.5	& 21.9	& 45.3	& 56.8\\
			& (c) TridentNet w/o scale-aware	& \checkmark &	\checkmark 	&   &	41.4    & 62.8  & 23.4	& 45.9	& \textbf{57.4}\\
			& (d) TridentNet w/o sharing & \checkmark &	&	\checkmark 			&   40.3	& 61.6	& 22.9	& 45.0	& 55.0\\
			& (e) TridentNet	& \checkmark &	\checkmark & \checkmark			&	\textbf{41.8}	& \textbf{62.9}	& \textbf{23.6} & \textbf{46.8} & 57.1 \\
		\hline						
	\end{tabular}
	\end{center}
\vspace{-3mm}	
\caption{Object detection results evaluated on the COCO \textit{minival} set~\cite{coco}. Starting from our baseline, we gradually add multi-branch design, weight sharing among branches and scale-aware training scheme in our TridentNet for ablation studies.}\label{tb:exp_ablation}
\end{table*}

First, we analyze the importance of each component in TridentNet. The baseline methods (Table~\ref{tb:exp_ablation}(a)) are evaluated on ResNet-101 and ResNet-101-Deformable~\cite{deformable} backbones. Then we gradually apply our multi-branch architecture, weight sharing design and scale-aware training scheme. 
\begin{enumerate}
\item \textbf{Multi-branch}. Based on the pilot experiment, Table~\ref{tb:exp_ablation}(b) evaluates a straightforward way to combine multiple branches of different dilation rates. This multi-branch variant improves over the baselines on AP for both ResNet-101 (from 37.9 to 39.0) and ResNet-101-Deformable (from 39.9 to 40.5), especially for large objects (2.3/1.2 increase). It indicates that even this simplest multi-branch design could benefit from different receptive fields.
\item \textbf{Scale-aware}. Table~\ref{tb:exp_ablation}(d) shows the ablation results of adding scale-aware training based on multi-branch (Table~\ref{tb:exp_ablation}(b)). It brings additional improvements (0.8/1.0 increase on ResNet-101/ResNet-101-Deformable) for small objects, but drops in performance for large objects. We conjecture that the scale-aware training design prevents each branch from training objects of extreme scales, but may also bring about over-fitting problem in each branch caused by reduced effective samples.
\item \textbf{Weight-sharing}. By applying weight sharing on multi-branch (Table~\ref{tb:exp_ablation}(c)) and TridentNet (Table~\ref{tb:exp_ablation}(e)), we could achieve consistent improvements on both two base networks. This demonstrates the effectiveness of weight-sharing. It reduces the amount of parameters and improves the performance of detectors. With the help of weight-sharing (Table~\ref{tb:exp_ablation}(e)), all branches share the same parameters which are fully trained on objects of all scales, thus alleviating the over-fitting issue in scale-aware training (Table~\ref{tb:exp_ablation}(d)). 
\end{enumerate}

Finally, TridentNets achieve significant improvements (2.7/1.9 AP increase) on the two base networks. It also reveals that the proposed TridentNet structure is compatible with methods like deformable convolution~\cite{deformable} which could adjust receptive field adaptively.

\end{paragraph}

\begin{paragraph}{Number of branches.}
We study the choice of the number of branches in TridentNets. Table~\ref{tb:nbranch_exp} shows the results using one to four branches. Note that we do not add scale-aware training scheme here to avoid elaborately tuning valid ranges for different number of branches. The results in Table~\ref{tb:nbranch_exp} demonstrate that TridentNets consistently improve over the single-branch method (baseline) with 2.7 to 3.4 AP increase. As can be noticed, four branches do not bring further improvement over three branches. Thus, considering the complexity and performance, we choose three branches as our default TridentNet setting.

\begin{table}[t]
\small
\renewcommand\arraystretch{1.25}
	\begin{center}
	%\setlength{\tabcolsep}{3.5pt}
	\begin{tabular}{c|cc|ccc}
		\hline
		Branches	& AP  & $\text{AP}_{50}$  & $\text{AP}_{s}$ & $\text{AP}_{m}$ & $\text{AP}_{l}$	\\
		\hline
		1 &  33.2	& 53.8	& 17.4	& 38.4	& 46.4 \\
		2 &  35.9	& 56.7	& \textbf{19.0}	& 40.6	& 51.2 \\
		3 &  \textbf{36.6}	& \textbf{57.3}	& 18.3	& \textbf{41.4}	& \textbf{52.3} \\
		4 &  36.5  & \textbf{57.3} & 18.8 & \textbf{41.4} & 51.9 \\
		\hline				
	\end{tabular}
	\end{center}
\vspace{-2mm}
\caption{Object detection results on the COCO \textit{minival} set~\cite{coco} using different number of branches on ResNet-50.% All results are based on ResNet-50 and share the same hyper-parameters.
}\label{tb:nbranch_exp}
\end{table}

\end{paragraph}

\begin{paragraph}{Stage of Trident blocks.}

We conduct ablation study on TridentNet to find the best stage to place trident blocks in ResNet. Table~\ref{tb:stage_exp} shows the results of applying trident blocks in conv2, conv3 and conv4 stages, respectively. The corresponding feature map strides are 4, 8 and 16 for the three stages. Comparing with conv4 stage, TridentNets on conv2 and conv3 stages achieve minor increase over the baseline. This is because the strides in conv2 and conv3 feature maps are not large enough to widen the discrepancy of receptive fields between three branches. %Thus the proposed trident blocks are successfully applied on conv4 stage to specialize each branch  with certain receptive field size. %scale through our scale-aware training strategy.

\begin{table}[t]
\small
\renewcommand\arraystretch{1.25}
	\begin{center}
	%\setlength{\tabcolsep}{3.5pt}
	\begin{tabular}{c|cc|ccc}
		\hline
		Stage	& AP  & $\text{AP}_{50}$  & $\text{AP}_{s}$ & $\text{AP}_{m}$ & $\text{AP}_{l}$	\\
		\hline
		Baseline &  33.2	& 53.8	& 17.4	& 38.4	& 46.4 \\
		\hline 
		conv2  &	  34.1	& 54.8	& 17.1	& 39.1	& 48.6  \\
		conv3  &  	  34.4  & 55.0  & 17.5	 & 39.3 & 49.0 \\
		conv4  &\textbf{36.6}	& \textbf{57.3}	& \textbf{18.3}	& \textbf{41.4}	& \textbf{52.3} \\
		\hline					
	\end{tabular}
	\end{center}
\vspace{-2mm}
\caption{Object detection results evaluated on the COCO \textit{minival} set~\cite{coco} by replacing conv blocks with trident blocks in different stages of ResNet-50.% All results are based on ResNet-50 and share the same hyper-parameters.
}\label{tb:stage_exp}
\end{table}

\end{paragraph}

\begin{paragraph}{Number of trident blocks.} 
As conv4 stage in ResNet has multiple residual blocks, we also conduct ablation study to explore how many trident blocks are needed for TridentNet. Here we replace different number of residual blocks with trident blocks on conv4 on ResNet-101. The results in Figure~\ref{fig:number_blocks} show that when the number of trident blocks grows beyond 10, the performance of TridentNet becomes stable. It indicates the robustness of TridentNet with regards to the number of trident blocks when the disparity of receptive fields between branches is large enough. 

\begin{figure}[hbpt]
\centering
\centering
\includegraphics[width=0.65\linewidth]{number_blocks}
\vspace{-1mm}
\caption{Object detection results on the COCO \textit{minival} set~\cite{coco} using different number of trident blocks on ResNet-101.}\label{fig:number_blocks}
%\vspace{-1mm}
\end{figure}

\end{paragraph}

\begin{paragraph}{Performance of each branch.}
\label{sec:exp_single} 
In this section, we investigate the performance of each branch of our multi-branch TridentNet. 
We evaluate the performance of each branch independently without scale-aware range constraints. 
Table~\ref{tb:branch_exp} shows the results of each single branch and three branches combined. 
As expected, through scale-aware training, branch-1 with the smallest receptive field achieves good results on small objects, branch-2 works well on objects with middle scale while branch-3 with largest receptive field is good at large objects. 
Finally, the three-branch method inherits the merits from three single branches and achieves the best results.
\end{paragraph}

\begin{table}[t]
\small
\renewcommand\arraystretch{1.25}
	\begin{center}
	\setlength{\tabcolsep}{3.5pt}
	\begin{tabular}{lc|cc|ccc}
		\hline
		Method & Branch No.	& AP  & $\text{AP}_{50}$  & $\text{AP}_{s}$ & $\text{AP}_{m}$ & $\text{AP}_{l}$	\\
		\hline
		Baseline & - & 	37.9	& 58.8	& {20.0}& {43.0}& 52.8\\
		\hline
		\multirow{4}{*}{TridentNet}		& Branch-1 & 31.5	& 53.9	& 22.0	& 43.3 & 29.9 \\
										& Branch-2 & 37.8	& 58.4	& 18.0	& 45.3 & 53.4 \\
										& Branch-3 & 31.9	& 48.8	& 7.1	& 37.9 & \textbf{56.1} \\
										& 3 Branches & \textbf{40.6}	& \textbf{61.8}	& \textbf{23.0} & \textbf{45.5} & 55.9 \\
		\hline
	\end{tabular}
	\end{center}
\vspace{-2mm}
\caption{Object detection results of each branch in TridentNet evaluated on the COCO \textit{minival} set~\cite{coco}. The dilation rates of three branches in Trident Network are set as 1, 2 and 3. The results are based on ResNet-101.% and share the same hyper-parameters.
}\label{tb:branch_exp}
\end{table}

\begin{table}[t]
\small
\renewcommand\arraystretch{1.25}
	\begin{center}
	\setlength{\tabcolsep}{3.5pt}
	\begin{tabular}{l|cc|ccc}
		\hline
		Scale-aware Ranges & AP  & $\text{AP}_{50}$  & $\text{AP}_{s}$ & $\text{AP}_{m}$ & $\text{AP}_{l}$	\\
		\hline
		(a) Baseline  & 	37.9	& 58.8	& {20.0}& {43.0}& 52.8\\
		\hline
		(b) $[0, 90], [30, 160], [90, \infty]$	 		& 37.8	& 58.4	& 18.0	& \textbf{45.3}  & 53.4 \\
		(c) $[0, 90], \enspace [0,  \infty], \enspace [90, \infty]$	 	& 39.3	& 60.1	& 19.1	& 44.6 & 56.4 \\
		(d) $[0, \infty], \enspace [0, \infty], \enspace [0, \infty]$  	& \textbf{40.0}	& \textbf{61.1}	& \textbf{20.9}	& 44.3	& \textbf{56.6} \\
		\hline
	\end{tabular}
	\end{center}
\caption{Object detection results of TridentNet Fast under different scale-aware range schemes evaluated on the COCO \textit{minival} set~\cite{coco}. All results are based on ResNet-101 and share the same hyper-parameters.}\label{tb:range_exp}
\end{table}
\end{subsection}

\begin{subsection}{Fast Inference Approximation}\label{sec:fast_infer}
To reduce the inference time of TridentNet, we propose TridentNet Fast which uses one major branch to approximate the three-branch results during inference. As indicated in Table~\ref{tb:branch_exp}, branch-2 emerges as a natural candidate for major branch as its scale-aware range covers most objects. We investigate the effect of scale-aware ranges for scale-aware training in Table~\ref{tb:range_exp}. As shown in Table~\ref{tb:range_exp}(c), by enlarging the scale-aware range of the major branch to incorporate objects of all scales, the performance of Trident Fast improves by 1.5 AP over the default scale-aware range setting. Furthermore, extending scale-aware ranges for all three branches achieves the best performance of 40.0 AP, which is close to the original TridentNet result of 40.6 AP. We hypothesize this may due to the weight-sharing strategy. Since the weights of the major branch are shared on other branches, training all branches in the scale-agnostic scheme is equivalent to do within-network multi-scale augmentation. 

\end{subsection}

\begin{subsection}{Comparison with State-of-the-Arts}\label{sec:results}

\begin{table*}[t]
\small
\renewcommand\arraystretch{1.25}
	\begin{center}
	%\setlength{\tabcolsep}{3.5pt}
	\begin{tabular}{ll|ccc|ccc}
		\hline
		Method &	Backbone	& AP  & $\text{AP}_{50}$  & $\text{AP}_{75}$ & $\text{AP}_{s}$ & $\text{AP}_{m}$ & $\text{AP}_{l}$	\\
		\hline
		% SSD513~\cite{ssd} & ResNet-101										& 31.2 & 50.4 & 33.3 & 10.2 & 34.5 & 49.8 \\
		% DSSD513~\cite{fu2017dssd}		&  ResNet-101						& 33.2 & 53.3 & 35.2 & 13.0 & 35.4 & 51.1 \\
		% RetinaNet~\cite{lin2017focal} & ResNet-101-FPN 						& 39.1 & 59.1 & 42.3 & 21.8 & 42.7 & 50.2 \\
		% hline
		% Faster R-CNN+++~\cite{resnet} & ResNet-101 							& 34.9 & 55.7 & 37.4 & 15.6 & 38.7 & 50.9 \\
		% Faster R-CNN w FPN~\cite{fpn} & ResNet-101-FPN 						& 36.2 & 59.1 & 39.0 & 18.2	& 39.0 & 48.2 \\
		% Faster R-CNN w FPN~\cite{fpn}\footnote{Detectron:\url{https://github.com/facebookresearch/Detectron/blob/master/MODEL_ZOO.md}} & ResNet-101-FPN \\
		Cascade R-CNN~\cite{cai2018cascade} 	& ResNet-101-FPN 			& 42.8 & 62.1 & 46.3 & 23.7	& 45.5 & 55.2 \\
		% Faster R-CNN by G-RMI~\cite{huang2017speed} & Inception-ResNet-v2   & 34.7 & 55.5 & 36.7 & 13.5 & 38.1 & 52.0 \\
		% Deformable R-FCN~\cite{deformable} & Aligned-Inception-ResNet-Deformable 		& 37.5 & 58.0 & 40.8 & 19.4 & 40.1 & 52.5 \\
		DCNv2~\cite{zhu2018deformable} & ResNet-101-DeformableV2                             & 46.0 & 67.9 & 50.8 & 27.8 & 49.1 & 59.5 \\
		% AttractionNet~\cite{gidaris2016attend} &  VGG16 + Wide ResNet 		& 35.7 & 53.4 & 39.3 & 15.6 & 38.0 & 52.7 \\
		DCR~\cite{cheng2018revisiting}			& ResNet-101-FPN-Deformable	& 43.1 & 66.1 & 47.3 & 25.8 & 45.9 & 55.3 \\
		SNIP~\cite{snip}	& ResNet-101-Deformable 						& 44.4 & 66.2 & 44.9 & 27.3 & 47.4 & 56.9 \\
		SNIPER~\cite{sniper}	& ResNet-101-Deformable 					& 46.1 & 67.0 & 51.6 & 29.6 & 48.9 & 58.1 \\
		\hline
		TridentNet						& ResNet-101						& 42.7 & 63.6 & 46.5 & 23.9 & 46.6 & 56.6\\
		TridentNet* 					& ResNet-101-Deformable 			& 46.8 & 67.6 & 51.5 & 28.0 & 51.2 & \textbf{60.5}\\ 
		TridentNet* + Image Pyramid	    & ResNet-101-Deformable	            & \textbf{48.4} & \textbf{69.7} & \textbf{53.5} & \textbf{31.8} & \textbf{51.3} & 60.3\\ 
		\hline

						
	\end{tabular}
	\end{center}
\vspace{-2mm}
\caption{Comparisons of single-model results for different object detection methods evaluated on the COCO \textit{test-dev} set~\cite{coco}.
%We perform inference with the major branch for TridentNets.
}\label{tb:results}
\end{table*}

In this section, we evaluate TridentNet on COCO \textit{test-dev} set and compare with other state-of-the-art methods. 
% In this part, we adopt ResNet-101 as our backbone network and increase the training epoch by 2$\times$ (3$\times$ for multi-scale training). 
% It is difficult to directly compare different detectors, since different methods may differ in backbone networks and training/test settings. 
%including image pyramid scheme~\cite{snip,sniper}, deformable convolutions~\cite{deformable}, large-batch Batch Normalization~\cite{peng2017megdet} and soft-NMS~\cite{softnms}. 
Here we report the results of our methods under different settings in Table~\ref{tb:results}.

TridentNet, which is to directly apply our method on Faster R-CNN with ResNet-101 backbone in the 2$\times$ training scheme, achieves 42.7 AP without bells and whistles. 

To fairly compare with SNIP and SNIPER, we apply multi-scale training, soft-NMS, deformable convolutions, large-batch BN and the 3$\times$ training scheme on TridentNet to get TridentNet*. 
It gives an AP of 46.8, already surpassing image pyramid based SNIP and SNIPER in the single-scale testing setting. 
If we adopt image pyramid for testing, it further improves the result of TridentNet* to 48.4 AP. 
To our best knowledge, for single models with ResNet-101 as backbone, our result is the best entry among state-of-the-art methods. %It shows that our TridentNet is compatible with these common techniques. 
Furthermore, TridentNet* Fast achieves 47.6 AP.


\begin{paragraph}{Compare with other scale handling methods.} 
In this section, we compare TridentNet with other popular scale handling methods like FPN~\cite{fpn} and ASPP~\cite{chen2017rethinking}. 
FPN is the \emph{de facto} model for handling scale variation in detection.
ASPP is a special case of TridentNet with only one trident block and dilation rates of three branches set to (6, 12, 18), followed by a feature fusion operator. 
To fairly compare with FPN, we adopt a \emph{2fc} head instead of a \emph{conv5} head for models in this section. 
Table~\ref{tb:fpn_compare} compares these methods under the same training setting. 
TridentNet improves significantly over other methods on all scales. 
It shows the effectiveness of scale specific feature maps generated by TridentNet with the same set of parameters. 
Furthermore, TridentNet Fast achieves 41.0 AP which still improves a lot over the compared methods.
{\let\thefootnote\relax\footnote{$^\dagger$Detectron: \url{https://github.com/facebookresearch/Detectron/blob/master/MODEL_ZOO.md}}}


\begin{table}[t]
\small
\renewcommand\arraystretch{1.25}
	\begin{center}
	\setlength{\tabcolsep}{3.5pt}
	\begin{tabular}{l|ccc|ccc}
		\hline
		Method &  AP  & $\text{AP}_{50}$  &  $\text{AP}_{75}$ & $\text{AP}_{s}$ & $\text{AP}_{m}$ & $\text{AP}_{l}$	\\
		\hline
		\emph{2fc} Baseline & 39.8 & 61.7 & 43.0 & 22.0 & 44.7 & 54.4 \\
		FPN$^\dagger$~\cite{fpn} & 39.8 & 61.3 & 43.3 & 22.9 & 43.3 & 52.6 \\
		ASPP & 39.7 & 60.4 & 42.7 & 21.7 & 44.5 & 53.9 \\
		TridentNet & \textbf{42.0} & \textbf{63.5} & \textbf{45.5} & \textbf{24.9} & \textbf{47.0} & \textbf{56.9} \\
		% TridentNet Fast & & & & & & \\
		\hline
	\end{tabular}
	\end{center}
\vspace{-2mm}
\caption{Comparisons of detection results on the COCO \textit{minival} set~\cite{coco}. Following FPN$^\dagger$, all methods are based on ResNet-101 with \emph{2fc} head using 2$\times$ training schedule.
}\label{tb:fpn_compare}
\end{table}


\end{paragraph}




\end{subsection}

\end{section}
